Link Prediction on Heterophilic Graphs via Disentangled Representation Learning

Link prediction is an important task that has wide applications in various domains. However, the majority of existing link prediction approaches assume the given graph follows homophily assumption, and designs similarity-based heuristics or representation learning approaches to predict links. However, many real-world graphs are heterophilic graphs, where the homophily assumption does not hold, which challenges existing link prediction methods. Generally, in heterophilic graphs, there are many latent factors causing the link formation, and two linked nodes tend to be similar in one or two factors but might be dissimilar in other factors, leading to low overall similarity. Thus, one way is to learn disentangled representation for each node with each vector capturing the latent representation of a node on one factor, which paves a way to model the link formation in heterophilic graphs, resulting in better node representation learning and link prediction performance. However, the work on this is rather limited. Therefore, in this paper, we study a novel problem of exploring disentangled representation learning for link prediction on heterophilic graphs. We propose a novel framework DisenLink which can learn disentangled representations by modeling the link formation and perform factor-aware message-passing to facilitate link prediction. Extensive experiments on 13 real-world datasets demonstrate the effectiveness of DisenLink for link prediction on both heterophilic and hemophiliac graphs. Our codes are available at https://github.com/sjz5202/DisenLink

==> Experiment.tex <==
\begin{table}[h]
\caption{The statistics of datasets}
\vskip -1em
\resizebox{1\linewidth}{!}{
\begin{tabular}{cccccc}
\hline
Dataset & Nodes &  Edges &  Features & Classes  & Edge hom. \\ \hline
Cora & 2,708 & 5,278 & 1,433 & 7 & 0.81 \\
CiteSeer & 3,327 & 4,552 & 3,703 & 6  & 0.74 \\
Photo & 7,650 & 238,162 & 745 & 8  & 0.82\\\hline
Chameleon & 2,277 & 36,101 & 2,325 & 5 & 0.23 \\ 
Squirrel & 5,201 & 216,933 & 2,089 & 5  & 0.22 \\
Crocodile & 11,631 & 180,020 & 500 & 6  &  0.25\\
Texas & 183 & 309 & 1,703 & 5  & 0.11 \\
Wisconsin & 251 & 499 & 1,703 & 5  & 0.20 \\
Twitch-ENGB & 7,126 & 36,324 & 2,545 & 2  & 0.55  \\
Twitch-DE & 9,498 & 153,138 & 2,514 & 2  & 0.63 \\
Johns Hopkins55 & 5,180 & 373,172 & 2406 & 2  & 0.50  \\
Amherst41 & 2,235 & 181,908 & 1,193 & 2  & 0.46 \\
%PubMed & 19,717 & 44,324 & 500 & 3 & Citation network & .80 \\
Arxiv-Year & 169,343 & 116,6243 & 128 & 40 & 0.22 \\ \hline
\end{tabular}
}
\label{tab:stat}
\end{table}

\section{EXPERIMENTS}
In this section, we evaluate the effectiveness of the proposed {\method} for link prediction on both homophilic and heterophilic graphs. Further analysis is provided to evaluate the influence of components in the proposed module. Specifically, we want to answer the following questions:
\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1} Can the proposed {\method}  with disentangled link reconstruction achieve outperformed accuracy for link prediction?
    \item \textbf{RQ2} How does each component in {\method} influence the effectiveness of link prediction?
    \item \textbf{RQ3} Does the {\method} with factor-wise neighborhood selection produce independent and distinguishable factors?
\end{itemize}

\subsection{Experiment Settings}
\subsubsection{Datasets} We conduct experiments on 13 publicly available benchmark datasets to evaluate the effectiveness of {\method} for link prediction performance. Among the 13 datasets, 3 of them are homophily graphs, i.e., Cora, CiteSeer and Photo, and the remaining 10 datasets are heterophilic graphs. These graphs are from various domains such as citation, Wikipedia and Amazon goods. We include both heterophilic and homophilic graphs of various domains to fully understand the effectiveness of {\method} for link prediction. The key statistics of the datasets are shown in Table~\ref{tab:stat}. The details of the datasets are given below: 
\begin{itemize}[leftmargin=*]
    \item \textbf{Cora} and \textbf{CiteSeer}~\cite{yang2016revisiting}: Both Cora and CiteSeer  are homophilic citation networks, where nodes represent documents and edges denote the citation relationships. The attributes of nodes are the bag-of-words representations of the papers. Cora has 2708 nodes and 5429 links. CiteSeer has 3327 nodes and 4715 links.%It contains one single graph with 2708 papers from 7 areas. There are 1433 attributes for each node and 5429 citation links for the whole graph.
    %\item \textbf{Citeseer}: Citeseer\cite{yang2016revisiting} is a homophily citation network similar with Cora. It contains one single graph with 3327 nodes. Each node has 3703 attributes and there is a total of 4715 citation links exist in the graph.
    \item \textbf{Photo}\cite{shchur2018pitfalls}: The Amazon Photo network is a homophilic goods network. Nodes denote goods and two connected nodes means that they are frequently bought together.  Node features are bag-of-words representation of goods' descriptions\suhang{I changed semantics to des, verify it}. It contains a graph with 7650 nodes with 8 classes and 238162 edges. The dimension of the feature is 745.
    \item \textbf{Texas and Wisconsin}~\cite{Pei2020Geom-GCN}: Texas and Wisconsin are heterophilic webpage networks collected from CMU, where nodes denote webpages and edges are the hyperlink connecting them. Node features are the bag-of-words representation of webpages. Texas contains 183 nodes with 5 classes and 309 edges and Wisconsin contains 251 nodes with 5 classes and 399 edges.
    %This network contains 183 nodes with 5 classes and 309 edges. The feature dimension is 1703.
    %This network contains 251 nodes with 5 classes and 399 edges. The feature dimension is 1703.
    \item \textbf{Chameleon, Squirrel and Crocodile}~\cite{Pei2020Geom-GCN}: Chameleon, Squirrel and Crocodile are heterophily Wikipedia page-page networks with each network on the topic denoted by its dataset name. Nodes are web pages and edges are hyperlinks between them. Each node's features denote several informative nouns in Wikipedia pages. The edge numbers range from 36101 to 360040 and the node numbers range from 2277 to 11631.  %It contains a graph with 2277 nodes.  The graph has 36101 links between the nodes.
    %\item \textbf{Squirrel}~\cite{Pei2020Geom-GCN}: Squirrel is a heterophily Wikipedia page-page network on squirrel topics. It is composed with the similar properties with Chameleon. It contains a graph with 5201 nodes. Each node has 2089 attributes. The graph has 217073 links between the nodes.
    %\item \textbf{Crocodile}~\cite{Pei2020Geom-GCN}: Crocodile is a heterophily Wikipedia page-page network on crocodile topics. It is composed with the similar properties with Chameleon. It contains a graph with 11631 nodes. Each node has 128 attributes. The graph has 360040 links between the nodes.
    \item \textbf{Facebook100}~\cite{traud2012social,lim2021new}: Facebook100 is composed of 100 Facebook friendship networks of American universities from 2005, where nodes represent students and edges denote friendship between students. Each node is labeled with gender. %The node numbers range from 769 to 41536. The link numbers range from 16656 to 1590655. 
    The node features are educational information of students. 
    We include two of them: \textbf{Johns Hopkins55} and \textbf{Amherst41} for our experiments.
    % \item Reed98: Reed98 is a friendship network from Facebook 100 networks. It contains one single graph with 962 nodes and 37624 links. For each node, its feature dimension is 745.
    \item \textbf{Twitch-explicit}~\cite{lim2021new}: twitch-explicit contains 7 networks where Twitch users are nodes and mutual friendships between them are edges. Node features are games liked, location and streaming habits. The node numbers range from 1912 to 9498. The link numbers range from 31299 to 153138. And the node feature dimensions range from 1288 to 2545. We include the two largest networks: \textbf{DE} and \textbf{ENGB} for our experiments.
    \item \textbf{arXiv-Year}~\cite{hu2020open}: arXiv-year is the ogbn-arXiv citation network with different labels. The nodes are arXiv papers and directed edges connect a paper to other papers that it cites. It contains a single graph with 169343 nodes and 1166243 links. The feature dimension is 128. We sample 10 subgraphs with around 5000 nodes and 15000 edges utilizing the RandWalk sampler in GraphSAINT~\cite{Zeng2020GraphSAINT}. \suhang{what do you mean? each subgraph contains 5000 nodes? The subgraphs are disconnected from each other}
\end{itemize}

\begin{table*}[h]
    \centering
    %\tiny
    % \vskip -0.5em
    \small
    \caption{Link Prediction performance (AUC(\%) $\pm$ Std.) on heterophilic graphs (``-'' denotes out of memory.)} \label{tab:heter}
    \vskip -1em
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lccccccccccc}
    \toprule
    Method & Chameleon &Squirrel & Crocodile & Texas & Wisconsin & Twitch-DE & Twitch-ENGB& Amherst41 & Johns Hopkins55 & Arxiv-Year \\
    \midrule
        AA & 95.8 $\pm 0.6$& 97.1 $\pm 0.4$& 90.6 $\pm 1.1$& 53.1 $\pm 6.2$& 61.5 $\pm 0.8$& 87.3 $\pm 0.2$&74.5 $\pm 0.4$&94.5 $\pm 0.7$&96.1 $\pm 0.5$&72.0 $\pm 0.9$\\
        CN & 95.3 $\pm 0.6$& 96.8 $\pm 0.4$& 89.8 $\pm 1.2$& 53.0 $\pm 6.2$& 61.3 $\pm 0.9$& 86.3 $\pm 0.1$&74.3 $\pm 0.2$&94.2 $\pm 0.6$&95.8 $\pm 0.6$&72.0 $\pm 0.9$\\
        SEAL&\textbf{99.5}$\pm0.1$&-&-&73.9 $\pm 1.6$&72.3 $\pm 2.7$&-& 90. &-&-&93.2$\pm0.8$&\\
        VGAE & 98.5 $\pm 0.1$ & 98.2 $\pm 0.1$ & 98.8 $\pm 0.1$ &68.6 $\pm 4.2$&71.3 $\pm 4.6$&84.3 $\pm 0.9$ &90.3 $\pm 0.2$& \textbf{97.2} $\pm 0.0$ & 92.8 $\pm 0.2$ &92.5 $\pm 0.5$  \\
        ARGVA & 96.5 $\pm 0.2$ & 93.6 $\pm 0.3$ & 94.1 $\pm 0.5$ &67.4 $\pm 6.1$&67.6 $\pm 3.0$&80.9 $\pm 1.1$&82.2 $\pm 0.8$& 81.2 $\pm 0.3$ &81.0 $\pm 0.7$  &86.8 $\pm 1.1$ \\
        GPR-GNN & 98.7 $\pm 0.1$ & 96.0 $\pm 0.3$ & 96.7 $\pm 0.1$ &76.3 $\pm 2.5$&80.1 $\pm 4.5$& 88.7 $\pm 0.1$&87.3 $\pm 0.1$& 93.7 $\pm 0.0$ & 94.7 $\pm 0.1$ & 93.0 $\pm 0.4$ \\
        FAGCN & 93.8 $\pm 2.6$ & 94.8 $\pm 0.3$ & 95.3 $\pm 0.2$ &68.7 $\pm 7.3$&73.7 $\pm 4.9$&85.4 $\pm 0.4$&89.6 $\pm 0.4$& 91.4 $\pm 0.3$  & 92.2 $\pm 0.3$  &84.8 $\pm 2.3$ \\
        LINKX & 98.8 $\pm 0.1$ & 98.1 $\pm 0.3$ & 99.0 $\pm 0.1$ &75.8 $\pm 4.7$&80.1 $\pm 3.8$&88.3 $\pm 1.9$&89.3 $\pm 1.6$& 93.5 $\pm 0.2$& 93.4 $\pm 0.3$ &88.4  $\pm 1.9$ \\
        GAT & 98.9 $\pm 0.1$ & 98.0 $\pm 0.0$ & 98.5 $\pm 0.1$ &68.5 $\pm 5.4$&68.1 $\pm 4.4$&87.4 $\pm 0.4$&86.1 $\pm 1.9$& 93.9 $\pm 0.1$ & 94.3 $\pm 0.5$ &92.5 $\pm 0.5$\\
        DisenGCN & 97.7 $\pm 0.1$ & 94.5 $\pm 0.2$ & 96.4 $\pm 0.4$ &72.1 $\pm 4.8$& 75.1 $\pm 3.4$&80.6 $\pm 0.2$&88.7 $\pm 0.3$& 87.9 $\pm 1.2$ & 90.7 $\pm 0.6$ &92.3 $\pm 0.5$\\
        FactorGCN & 98.3 $\pm 0.3$ & 96.9 $\pm 0.4$ & 97.6 $\pm 0.4$ &58.7 $\pm 4.1$&68.8 $\pm 9.0$&87.2 $\pm 0.7$&89.8 $\pm 0.6$& 91.5 $\pm 0.7$ & 92.3 $\pm 0.4$ & 90.5 $\pm 1.0$ \\
        \midrule
        {\method} &\textbf{99.4} $\pm 0.0$ & \textbf{98.3} $\pm 0.1$ &  \textbf{99.1} $\pm 0.1$ &\textbf{80.7} $\pm 4.0$&\textbf{84.4} $\pm 1.9$&\textbf{93.7} $\pm 0.1$&\textbf{96.2} $\pm 0.1$& \textbf{97.2} $\pm 0.0$ & \textbf{97.5} $\pm 0.1$ &\textbf{95.0} $\pm 0.3$\\
        \bottomrule
    \end{tabular}
     }
    
    %\vskip -0.5em
\end{table*}

\subsubsection{Baselines} We include classical heuristics, GNN based link prediction method, GNN based representation learning methods for link prediction, disentangled GNNs and GNNs for heterophilic graphs as our baselines. For baselines without the link prediction module , they are performed as encoders in the VGAE manner. Here is a brief introduction of each baseline:
\begin{itemize}[leftmargin=*]
    \item \textbf{CN}: Common-neighbor index is a classical link prediction method based on connectivity, which assumes that two nodes are more likely to connect if they have many common neighbors.
    \item \textbf{AA}~\cite{adamic2003friends}: Adamic–Adar index is a second-order heuristic based on the assumption that a shared neighbor with large degree is less significant to the measure of a link.
    \item \textbf{VGAE}~\cite{alemi2016deep}: Variational Graph Autoencoder is a generative model for graph representation. Here we use a GCN with two 2-layer encoder shared the first hidden layer\suhang{?????} and a link reconstruction module as the decoder.
    \item \textbf{ARGVA}~\cite{pan2018adversarially}: Adversarially Regularized Variational Graph Autoencoder  is inspired by the adversarial learning methods and the latent representation is enforced to match a prior distribution via an adversarial training scheme.
    \item \textbf{GPR-GNN}~\cite{chien2020adaptive}: Generalized PageRank GNN adaptively learns the GPR weights to optimize the node representation, regardless of the homophilic graph or heterophilic graph.
    \item \textbf{FAGCN}~\cite{bo2021beyond}: Frequency Adaptation Graph Convolutional Networks utilizes a selfgating mechanism to adaptively integrate different signals in the process of message passing.
    \item \textbf{LINKX}~\cite{lim2021large}: Linkx decoupled the feature representation and structure representation and use a simple framework to process the decoupled information.
    \item \textbf{GAT}~\cite{velivckovic2017graph}: GAT is a message-passing graph neural network utilizing attention mechanism for better aggregation of neighborhood.
    \item \textbf{DisenGCN}~\cite{ma2019disentangled}: DisenGCN learn disentangled node representations and then utilizes a novel neighborhood routing mechanism to find latent factors that shapes the relationship between the nodes. Then for each factor the nodes aggregate the information and get different representations.
    \item \textbf{FactorGCN}~\cite{yang2020factorizable}: FactorGCN shares the similar motivation of disentangling graphs with respect to latent factors. And this models focus more on graph-level tasks.
    \item \textbf{SEAL}~\cite{zhang2018link}: SEAL is a link prediction method that use a GNN to learn heuristics from local subgraphs automatically.
\end{itemize}
\subsubsection{Configurations} We use a 64-bit machine with Nvidia GPU (Tesla V100, 1246MHz , 32 GB memory) to conduct our experiments. We use ADAM optimization algorithm to train the models. For all methods, the learning rate is initialized to 0.001, with weight decay being 5e-4. We train all the models until converging with a maximum training epoch 2000.

\subsubsection{Evaluation Metrics} Following existing works~\cite{}\suhang{cite} in evaluating link prediction, area under the curve (AUC) is used as our evaluation metrics to measure the prediction accuracy.
\suhang{can you state the details of your evaluation. you mentioned last time that following a paper, for each positive link, you sampled xx negative samples to form a data sample or something, you then calculate AUC for each one?}

\subsubsection{Implementation Details}
Edges in each dataset are split into 3 parts: 85\% for training, 5\% for validation and 10\% for testing. \suhang{how many times did we do the split, just once?} \suhang{state that the hyperparameters of all methods are searched on xxxx} For {\method}, the temperature parameter $\tau$ v is varied among $\{0.1,1\}$ and the teleport parameter $\beta$ is varied from 0.1 to 0.9.\suhang{number of latent factors}

\subsection{Link Prediction Performance}

\begin{table}[h]
    \centering
    %\tiny
    % \vskip -0.5em
    \small
    \caption{Link Prediction performance (AUC(\%) $\pm$ Std.) on homophilic graphs (``-'' denotes out of memory.)} \label{tab:homo}
    \vskip -1em
    %\resizebox{0.75\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    Method & Cora & Citeseer & Photo \\
    \midrule
        AA & 75.9 $\pm 1.5$ & 69.8 $\pm 2.2$& 97.4 $\pm 0.4$\\
        CN & 75.7 $\pm 1.3$ &69.7$\pm 2.3$&97.1 $\pm 0.4$\\
        SEAL &90.4 $\pm 1.1$& 97.0 $\pm 0.5$&-\\
        VGAE & 96.6 $\pm 0.2$ & 97.3 $\pm 0.2$ & 94.9 $\pm 0.8$ \\
        ARGVA & 92.7 $\pm 1.3$ & 94.8 $\pm 0.4$& 89.7 $\pm 2.3$ \\
        GPR-GNN & 94.8 $\pm 0.3$ & 96.0 $\pm 0.3$ & 97.0 $\pm 0.2$\\
        FAGCN & 91.8 $\pm 3.4$ & 89.2 $\pm 5.6$& 94.0 $\pm 1.9$\\
        LINKX & 93.4 $\pm 0.3$& 93.5 $\pm 0.5$& 97.0 $\pm 0.2$\\
        GAT & 97.0 $\pm 0.2$ &  \textbf{98.3} $\pm 0.2$& 97.3 $\pm 0.3$\\
        DisenGCN & 96.6 $\pm 0.3$ & 96.8 $\pm 0.2$& 95.2 $\pm 1.3$\\
        FactorGCN & 92.3 $\pm 1.4$ & 87.8 $\pm 3.6$ & 97.2 $\pm 0.1$\\
        \midrule
        {\method} & \textbf{97.1} $\pm 0.4$ &  \textbf{98.3} $\pm 0.3$& \textbf{97.9} $\pm 0.1$ \\
        \bottomrule
    \end{tabular}
`     %}
    
    %\vskip -0.5em
\end{table}
To answer \textbf{RQ1}, we evaluate the link prediction performance of {\method} with comparison  on 10 heterophilic and 3 homophilic graphs. Each experiment is repeated 5 times to alleviate randomness. The average link prediction performance measured by AUC with standard deviations on heterophilic graphs and homophilic graphs are shown in Table~\ref{tab:heter} and Table~\ref{tab:homo}, respectively. From tables, we have the following observations: \suhang{the analysis is too long. may need to merge some items if we don't have enough space}
\begin{itemize}[leftmargin=*]
\item Compared with classical heuristics AA and CN, our method outperforms them in all datasets. For Wikipedia, FB100 and Photo datasets with higher average node degree, the performance gap is relatively small. While AA and CN only rely on the graph structural feature, for the other datasets with smaller average node degree, {\method} is much  better due to the disentangled learning of both node features and the graph structure.
\item {\method} has comparable performance on the Chameleon and outperforms other datasets compared with SEAL. It needs to be noticed that SEAL fails to be implemented on graphs with large number of edges which will leads to the huge memory consuming of the enclosing subgraph extraction before learning, while {\method} is implemented in a end-to-end fashion.
\item Compared with unsupervised representation learning methods VGAE and ARGVA\suhang{they are not unsupervised representation learning, they have supervised link prediciton loss}, {\method} performs better and is much more robust across datasets as there is a larger performance gap between similar datasets in VGAE (DE and ENGB, Amberst41 and Johns Hopkins55). For ARGVA, the adversarial training does not fit well for the link prediction task. Compared with the GCN encoder in them, the modeling of edge factors in {\method} disassembles the complex edge relationships in heterophilic graphs for the better structural information mining.
\item For state of the art GNNs targeted for heterophilic graphs GPR-GNN,FAGCN and LINKX, performing as a encoder in VGAE, they perform worse in heterophilic datasets, e.g. crocodile, ENGB, compared with vanilla VGAE. Although these methods can successfully improve the node feature learning respect to the node classification task for heterophilic graphs, they fail to capture different latent relations underlying graph structure using the same set of learnt representations. {\method} can better preserve different relational information via separated link reconstruction for different factors and thus outperform these heterophilic graph targeted methods.
\item {\method} also perform better than other disentangled GNN methods and GAT in link prediction. For disentangled GNN models DisenGCN and FactorGCN, they perform factor-wise message-passing with the same graph structure. Although node representations are weighted differently in each factor, the unrelated nodes in each factor will still add unnecessary signals when aggregated with the nodes pertinent to that factor. In contrast, {\method} performs individual message-passing with disjoint adjacency matrix and merge the learnt structural information by the proposed disentangled link reconstruction at the end. GAT have good performance and even perform better on Citeseer than {\method} thanks to its multi-head attention mechanism.
\item In general, {\method} can be adapted well both on small and large graph datasets. For small graph Texas and Wisconsin, {\method} shows apparent improvement around 10\% compared with baselines. For large graph dataset Arxiv-Year, besides better accuracy, {\method} is more stable with smaller standard variance because the factor-aware neighbor selection can adaptively formulate disjoint factors that fit the dataset.
\end{itemize}
In summary, these results verify the advantage of unsupervised link prediction\suhang{it's not unsupervised link prediction, it's supervised, fix all these} with the disentangled manner. Compared with baselines with different specific characteristics, e.g. disentangled model, GNNs for heterophilic graphs, {\method} exhibit comprehensive learning capacity for link prediction due to the factor-aware neighbor selection, factor-wise message-passing and disentangled link reconstruction. %We will do further ablation study in next section to analyze each component in our proposed method {\method}.
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/ablation.png}
    \vskip-1em
    \caption{Affect of different components in {\method}}
        \label{fig:ablation}
    %\vskip 1em
\end{figure}
\subsection{Ablation Study}
In this section,in order to answer the \textbf{RQ2}, we put forward experimental analysis to evaluate the effect of each component in our model. Each ablation experiment is conducted 5 times to alleviate the randomness.

\textbf{Importance of the disentangled manner} We first examine the advantage of the disentangled learning manner compared with the normal model with a single factor. Shown in the Fig.~\ref{fig:nfactor}, model with multiple factors perform much better than the model with single factor, especially in the case of heterophilic graph ENGB. It proves that the disentangled representation can facilitate more effective egde relation discovery compared with normal learning.

\textbf{Significance of the factor-wise importance value} Secondly, the importance value $\alpha$ computed from Eq.~{\ref{eq:attention}} for message passing is crucial for link prediction on heterophilic graphs. In the case of ENGB in Fig.~{\ref{fig:engb_nfactor1}}, we can observe that even without disentanglement, the performance of {\method} is much better than VGAE. This is because the $\alpha$ weights representations in the message-passing process to leverage each neighbor node's affect according to the importance/similarity $\alpha$. Compared with the performance of GAT which include the multi-head attention mechanism similar with $\alpha$, the single factor {\method} also has much better accuracy which reflect the concatenation operation for multi-head attention and output representation computing in GAT can not effectively preserve the relational information for link prediction on heterophilic graphs.
We also remove all the $\alpha$ involved in {\method} to formulate the model variant {\methoda}. Compared with {\method}, the performance of {\methoda} shown in Fig.~{\ref{fig:ablation}} is much lower in all datasets. It demonstrates the importance of relational weighting in message-passing and link reconstruction for link prediction.  

\textbf{Influence of the factor-aware neighbor selection}We also conduct ablation study to explore the influence from the factor-aware neighbor selection on the link prediction on heterophilic graphs. The comparative experiment is between {\method} and the variant {\methods} without the proposed factor-aware neighbor selection, i.e. the neighborhood of node s $\mathcal{N}_{s, k}$ for each factor in {\methods} becomes same as $\mathcal{N}_{s}$. In this case, from the Fig.~{\ref{fig:ablation}}, {\method} outperforms {\methods} which reflects the selection of the most important factor between two node to formulate K disjoint neighborhoods is very helpful for link prediction.

\textbf{Influence from link reconstruction manner of {\method}} In {\method}, the link reconstruction utilizing the learnt disentangled representation is implemented as Eq.~{\ref{eq:re}}. Here, we compare it with the vanilla manner in VGAE~{\cite{kipf2016variational}} combined with disentangled representation as Eq.~{\ref{eq:link_prediciton_equally}}. This model variant is named as {\methodr}. The performance difference between them shown in the Fig.~{\ref{fig:ablation}} verifies the effectiveness of our disentangled link reconstruction which o assign different factors with different importance during link prediction


\begin{figure}
\centering
\subfigure[Cora]{
    %\centering
    \includegraphics[width=0.50\linewidth]{figure/out_cora.png}
    \label{fig:cora_nfactor}
}\subfigure[ENGB]{
    %\centering
    \includegraphics[width=0.50\linewidth]{figure/out_engb.png}
    \label{fig:engb_nfactor}
}
\caption{Performance of our model with different number of factors,\suhang{make the font size larger, add subcation}\shijie{should we add one baseline horizontal line, e.g. VGAE in each of them?like following in Fig.~{\ref{fig:nfactor1}}}}
\label{fig:nfactor}
\end{figure}
\begin{figure}
\centering
\subfigure[Cora]{
    %\centering
    \includegraphics[width=0.50\linewidth]{figure/out_cora_withb.png}
    \label{fig:cora_nfactor1}
}\subfigure[ENGB]{
    %\centering
    \includegraphics[width=0.50\linewidth]{figure/out_engb_withb.png}
    \label{fig:engb_nfactor1}
}
\vskip -1em
\caption{Performance of our model with different number of factors (the red line denotes the performance of VGAE)}
\label{fig:nfactor1}
\end{figure}
\begin{figure}[h]
\centering
    \includegraphics[width=0.85\linewidth]{figure/beta.png}
    \vskip -1em
    \caption{Parameter Sensitivity of $\beta$ }     \label{fig:beta}
    %\vskip 1em
\end{figure}
\subsection{Parameter Sensitivity Analysis}
In this section, we investigate the sensitivity of {\method}'s performance respect to two hyper-parameters: the number of factors K and the $\beta$ in message passing. For the number of factors K, we vary it from 1 to 10 and conduct the experiments on one homophilic graph Cora and one heterophilic graph ENGB as shown in Fig.~\ref{fig:nfactor}. Hyper-parameter $\beta$ is varied from 0 to 1 and the experiment of $\beta$ shown in Fig.~\ref{fig:beta} is conducted on Cora, ENGB and ArXiv-year with fixed K.

According to the Fig.~\ref{fig:cora_nfactor}, when the number of factors equal to 8 which is a slightly bigger than its actual numbers of ground truth 7, experiments on Cora reach the best performance. For ENGB which has 2 ground truths, the performance reaches the peak around $k=6$ and fluctuates slightly after it shown in Fig.~\ref{fig:engb_nfactor}. This is bacause the number of ground truth can not reflect the actual number of latent factors in hetrophilic graphs due to the complex intra-class distribution. 

The sensitivity of $\beta$ shown in Fig.~\ref{fig:beta} reflect how the proportion of the central node content in factor-wise message-passing affects the link prediction. The existence of $\beta$ can help the preservation of locality and prevent uninformative node representation in each factor since the disjoint factor graph includes isolated nodes. As a result,when $\beta> 0$, the performance will be much improved. And when $\beta$ is near 1, the performance will drop due to the lack of neighbor feature information.
\begin{figure}
\centering     
\subfigure[The representation correlation of {\methods}]
{\label{fig:corre_without}
\includegraphics[width=0.98\linewidth]{figure/feature_corr_5fatcor_data_naive.png}}
\vskip -1em
\subfigure[The representation correlation of {\method}]
{\label{fig:corre_with}
\includegraphics[width=0.98\linewidth]{figure/feature_corr_5fatcor_data.png}}
\vskip -1em
\caption{Disentangled feature correlation coefficient without/with proposed module}
%\vskip -1em
\label{fig:coeffcient}
\end{figure}




% \begin{figure}[t]
% \centering
% \subfigure[without proposed module]{
% \begin{minipage}[t]{0.50\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figure/feature_corr_5fatcor_data_naive.png}
% %\caption{fig1}
% \end{minipage}%
% }%
% \subfigure[with proposed module]{
% \begin{minipage}[t]{0.50\linewidth}
% \centering
% \includegraphics[width=\textwidth]{figure/feature_corr_5fatcor_data.png}
% %\caption{fig2}
% \end{minipage}%
% }%

% \centering
% \vspace{-4mm}
% \caption{Disentangled feature correlation coefficient without/with proposed module\suhang{why the subcaption is so strange, there should be (a) (b) pop up automatically}}
% \label{fig:coefficient}
% \vspace{-3mm}
% \end{figure}

\subsection{Case Study/Visualization}
In this section,we compute the absolute value of the correlations between the elements of the 160-dimensional node representations from {\method} and the model variant {\methods} in which all factors share the same graph structure. Both of them are setted with five factors. We visualize them in Fig.~{\ref{fig:coeffcient}}. Compared with the mixed correlation in the case of {\methods} shown in Fig.~{\ref{fig:corre_without}}, the correlation plot of {\method} in Fig.~{\ref{fig:corre_with}} shows 5 explicit blocks in the diagonal. The difference between {\method} and {\methods} implies the factor-aware neighbor selection can produce independent factors and promote the disentanglement of the output representations which can be an answer of \textbf{RQ3}.
\section{CONCLUSION AND FUTURE WORK}

\begin{table*}[t]
    \centering
    %\tiny
    % \vskip -0.5em
    \small
    \caption{Full list of Link Prediction performance (AUC(\%) $\pm$ Std.) on the Twitch-e Dataset} \label{tab:heter1}
    % \vskip -1em
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    Method & Twitch-RU & Twitch-ENGB & Twitch-ES & Twitch-PTBR & Twitch-TW & Twitch-FR & Twitch-DE  \\
    \midrule
        VGAE & 89.0 $\pm 0.2$ & 90.3 $\pm 0.2$ & 89.7 $\pm 0.4$ & 87.0 $\pm 0.6$ & 86.7 $\pm 0.6$ & 87.2 $\pm 0.4$ & 84.3 $\pm 0.9$ \\
        ARGVA & 79.5 $\pm 1.4$ & 82.2 $\pm 0.8$ & 82.8 $\pm 0.7$ & 77.7 $\pm 1.0$ & 77.1 $\pm 0.3$ & 75.4 $\pm 0.7$ & 74.9 $\pm 0.4$\\
        GPR-GNN & 87.5 $\pm 1.0$ & 87.3 $\pm 0.1$ & 90.4 $\pm 0.2$ & 88.4 $\pm 0.9$ & 89.0 $\pm 1.3$ &90.0 $\pm 0.1$ &88.7 $\pm 0.1$\\
        FAGCN & 88.4 $\pm 0.5$ & 89.6 $\pm 0.4$ & 89.6 $\pm 0.5$ & 87.3 $\pm 0.3$  & 87.4 $\pm 0.3$ & 87.1 $\pm 0.5$  & 85.4 $\pm 0.4$\\
        LINKX & 90.9 $\pm 0.3$ & 89.3 $\pm 1.6$ & 91.3 $\pm 0.2$ & 90.9 $\pm 0.8$ & 90.7 $\pm 0.3$ & 90.5 $\pm 0.3$ & 88.3 $\pm 1.9$\\
        GAT & 85.8 $\pm 2.8$ & 86.1 $\pm 1.9$ & 87.6 $\pm 1.2$ & 85.7 $\pm 2.3$ & 88.2 $\pm 0.8$ & 87.8 $\pm 1.3$ & 87.4 $\pm 0.4$\\
        DisenGCN & 83.9 $\pm 1.9$ & 88.7 $\pm 0.3$ & 86.2 $\pm 1.6$ & 78.1 $\pm 4.1$ & 78.3 $\pm 2.9$ & 81.6 $\pm 1.3$& 80.6 $\pm 0.2$\\
        FactorGCN & 87.7 $\pm 1.0$ & 89.8 $\pm 0.6$ & 89.6 $\pm 0.9$ & 87.3 $\pm 2.3$ & 87.9 $\pm 0.3$ & 88.2 $\pm 1.5$ & 87.2 $\pm 0.7$\\
        \midrule
        Ours & \textbf{95.4} $\pm 0.2$ & \textbf{96.0} $\pm 0.1$ &  \textbf{95.6} $\pm 0.6$ & \textbf{95.0} $\pm 0.1$ & \textbf{95.1} $\pm 0.2$ & \textbf{95.2} $\pm 0.1$ & \textbf{93.7} $\pm 0.1$\\
        \bottomrule
    \end{tabular}
    }
    \vskip -0.5em
\end{table*}

==> Introduction.tex <==
\section{Introduction}

In the real world, the relational information between individual contents and identifications builds links between them and thus formulates the ubiquitous graph structured data. However, there exists many unknown and potential links in real-world graphs due to the limitation of observation capacity, artificial masking, .etc. It have aroused increased research on the link prediction task in practical applications such as social network recommendation~\cite{yang2018graph}, the completion of knowledge graph ~\cite{Nickel2016ARO}, protein–protein interaction reconstruction ~\cite{lei2013novel}. 

Some previous research on link prediction focused on heuristic methods such as common neighbors(CN), Adamic-Adar (AA)~\cite{adamic2003friends}, SimRank (SR)~\cite{jeh2002simrank}. These methods are strongly rely on corresponding connectivity assumption or a specific intuitive graph theory. However, despite their simplicity and effectiveness in some graphs, heuristic would fail when the input graph contradicts the underlying assumption. For example, SimRank based link prediction depends on the assumption that similar nodes share similar neighborhoods which may work on homophlic graphs. But in heterophilic graphs where nodes with unsimilar attributes and features tend to be linked, neighbor distribution is far more complex and thus the connectivity between a pair of nodes can not be affirmed correctly under SimRank's assumption. Besides heuristic methods, Graph neural networks (GNNs) based link prediction methods such as VGAE~\cite{kipf2016variational},SEAL~\cite{zhang2018link} successfully achieved state-of-the-art performance. But in both cases, they rely on a Graph Convolutional Network (GCN)~\cite{kipf2016semi} to capture the topology and feature information under the homophily assumption which also conflicts the disassortativity in real-world graphs. 
\begin{figure}[t]
\centering
    \includegraphics[width=0.8\linewidth]{figure/heterophilic.pdf}
    \vskip -1em
    \caption{Example of heterophilic graphs. (We use color to denote different node pairs.) There may exist many latent factors that cause the formation of links. For this graph, if we aggregate information from neighbors, there will be much noise from neighbor nodes since all the factors are mixed up. In our model, we disentangle all the factors and propagate them separately.}     \label{heterophilic}
    \vskip -1em
\end{figure}

In real-world graphs such as social networks, taking Fig.~{\ref{heterophilic}} as an example , we use nodes to represent members in the social network and the connection between two nodes can represent various kinds of relationships and thus takes into multiple latent factors. For example, two nodes are connected because they are colleagues; while another pair of nodes are connected because they are fans of music. Because of various latent factors causing the formation of links, the formed graph may not necessarily follow the homophily assumption. They fail to generalize to heterophilic graphs where linked nodes may have dissimilar labels and attributes. That means, two nodes with “colleague” relationship could have totally different cultural backgrounds and interests, making their attributes very dissimilar. Thus, directly performing message passing on such heterophilic graphs could aggregate neighbors of dissimilar features of the center nodes, causing noisy representations~\cite{bo2021beyond} which even degrade link prediction performance compared with the heuristics only based on graph topology. 

Under this scenario that a central node is connected with diverse latent factors, factorizing the entangled central node's representation to the disentangled representation is the antidote to extract unmixed link relations. Previous research has also shown that disentangled representations are more resilient to the complex variants~\cite{bengio2013representation}, and capable to generalize well on different tasks~\cite{alemi2016deep}.  Thus, in our work, we carry out the link prediction in the disentangled learning manner, i.e. learning disentangled node representations from GNNs for link prediction in heterophilic graphs. 

Previous disentangled learning methods on graphs have succeeded in node\cite{ma2019disentangled} and graph\cite{yang2020factorizable} classification. When it comes to the link prediction on heterophilic graphs, several challenges remain to be solved: (i)  How to learn high-quality disentangled representations that capture the most informative and pertinent latent factor without supervision of latent factor selection? (ii) How to model link formation of representations from multiple factors? (iii) how can we learn the disentangled representations that capture the neighborhood information beyond the noisy aggregation in real-world heterophilic graphs for better link predictions?

To address these challenges, in this work, we propose a link prediction model named {\method}. {\method} focus on edge factor discovery at the beginning to select the most important edge factor for each potential connectivity based on the similarity between local representations for informative factors. {\method} then takes the relational similarity information and graph locality into consideration and perform factor-wise message passing within the neighbor of selected factor to produce disentangled representations for better link prediction. {\method} doesn't naively reconstruct links following VGAE~\cite{kipf2016variational} but consider the different contributions of each factor and thus propose the factor-wise link reconstruction for final prediction. In summary, this work makes the following main contributions:
\begin{itemize}
\item We rethink and solve the link prediction task from the view of disentangled learning.
\item We propose factor-wise message passing with factor-aware neighbor selection  to promote to encourage high-quality disentanglement.
\item We successfully improve the effectiveness of {\method} both on heterophilic and homophilic graphs.
\end{itemize}

%The ubiquity of graph structured data involved in real-world problem:  such as social network recommendation~\cite{yang2018graph}, the completion of knowledge graph ~\cite{Nickel2016ARO}  have aroused prevalent needs for the graph representation learning method. Graph neural network (GNNs) has become a clear answer for the graph representation learning as GNNs can efficiently extract graph topology and node/edge attributes information via message-passing mechanism both in spectral~\cite{kipf2016semi} and spacial~\cite{hamilton2017inductive} manners. Graph neural networks have achieved remarkable success in downstream tasks and are going through rapid development over these years~\cite{wu2020comprehensive}.

%Although GNNs have addressed many real-world problems successfully, most GNNs design their message-passing mechanisms based on the homophily assumption of graphs~\cite{zhu2020beyond}, which generally assumes that two connected nodes share similar features or node attributes. In real-world graphs such as social networks, we use nodes to represent members in the social network and the connection between two nodes can represent various kinds of relationships and thus takes into multiple latent factors. For example, two nodes are connected because they are colleagues; while another pair of nodes are connected because they are fans of music. Because of various latent factors causing the formation of links, the formed graph may not necessarily follow the homophily assumption. They fail to generalize to heterophilic graphs where linked nodes may have dissimilar labels and attributes. That means, two nodes with “colleague” relationship could have totally different cultural backgrounds and interests, making their attributes very dissimilar. Thus, directly performing message passing on such heterophilic graphs could aggregate neighbors of dissimilar features of the center nodes, causing noisy representations which degrade the performance of downstream tasks~\cite{bo2021beyond}. \suhang{design a figure to show that (i) in heterophilic graphs, there are many latent factors that causes the formation of a link instead of the simple homophily assumption, and two nodes are connected due to one or two latent factors (ii) the heterophilic graph challenges link prediction and message-passing; and (iii) if we can learn disentangled representation and model the latent factors, we can learn better representation to better predict missing links}




% heterophilic -> disentangled (motivation)
%Recently, researchers propose the idea of disentangled representation learning to learn the latent factors behind the data separately in computer vision. Researchers find such representations are more resilient to the complex variants~\cite{bengio2013representation}, and capable to generalize well on different tasks~\cite{alemi2016deep}. 
%Inspired by the recent development of disentangled graph neural  networks~\cite{ma2019disentangled}, we aim at leveraging the disentangled representation on link prediction tasks to mitigate the heterophilic graph learning issues. 
%However, incorporating disentanglement node representation into unsupervised heterophilic graph learning is a difficult task~\cite{zhao2022exploring}. There are two main challenges in learning disentangled representation: (i) there is no ground-truth of the factors shared by two nodes. Thus, how can we design self-supervision to provide signals for disentangled representation learning; and (ii) how to effectively perform the factor-wise message-passing?

%To address these challenges, in our work, we focus on facilitating graph representation learning, particularly the link prediction tasks, with multi factors among the nodes. We propose a factor-wise message-passing module, and make attempts to design a set of pretext tasks to guide the disentangled representation learning for nodes. Our approach enables node representations to learn the latent factors among different pairs of nodes. Concretely, we project each node to a set of factors to get the disentangled representation and perform the message-passing for different factors separately. And we leverage a set of self-supervision pretext tasks to help to capture the structure information and feature information residing in the data. With the disentangled representation, we perform link prediction tasks on test set. Compared with previous works, our model is capable to model multi latent factors and get disentangled representation of nodes. Finally, extensive experiments will be performed on public datasets. We expect the results can outperform other methods to demonstrate the superiority of our method.

%In summary, this work makes the following main contributions:
%\begin{itemize}
%    \item We
%\end{itemize}

==> Methodology.tex <==
\section{METHODOLOGY}
In this section, we will give the detailed of the proposed framework {\method} to learn disentangled node representations for link prediction on heterophilic graphs. The core idea of {\method} is: for each nodes $v_s$, we want to learn $K$ disentangled representation vectors $[\mathbf{z}_{s,1}, ..., \mathbf{z}_{s,K}]$ including multiple distinguishable embeddings learnt from $K$ latent factors and utilize the learnt representations to do the message-passing and aggregation on each factors individually. Node representations from all latent factors are incorporated together to participate into the graph structural reconstruction for the link prediction task. Several challenges left for us to addressed: (i) while no ground truth of each factor is pre-defined in the disentangled learning, extra discriminator with self-defined ground-truth or loss from the measure of covariance between disentangled channels are involved in some previous works to encourage and improve disentanglements. How to encourage the independence and improve the informativeness among the latent factors in the more efficient manner with simplicity? (ii) Since the dissimilar neighbor feature aggregation in heterophilic graphs causes noisy representation of the central node, how to mitigate the noisy aggregation via better neighbor candidates selection? (iii) With little dependence on the homophily assumption, in heterophilic graphs, the bond between edge semantic information and graph topology is fragile and thus there exists less trustworthy predictions from the link reconstruction output. Since disentangled representations address this issue by extracting different relational information factor-wisely, how can the individual embeddings in each factor be incorporated for united link reconstructions? To address these challenges, besides initial factor-wise feature projection via simple multilayer perceptron, the framework of our {\method} consists another 3 parts: 1.factor-wise importance matrix and related neighbor candidates selection, 2.relational neighbor aggregation with leveraged revisit and 3.disentangled link reconstruction for self-supervision. The detailed introduction is following.
\begin{figure*}
    \centering
    \includegraphics[width=0.85\linewidth]{figure/model1.pdf}
    \vskip -1em
    \caption{The overview of the framework\suhang{make font larger}}
    \label{fig:model}
\end{figure*}
\subsection{Neighbor Selection via Factor-wise Importance Matrix}
{\method} includes K factors. For each node $v_s$, we first project its feature to the $k$-th factor as $\mathbf{z}_{s,k}=f_k(\mathbf{x}_{s})$, where $f_k$ is a function such as MLP:
\begin{equation} \label{eq:mlp}
\mathbf{z}_{s,k}=\mathbf{W}_k^{(2)}ReLU(\mathbf{W}_k^{(1)}\mathbf{x}_{s})
\end{equation}
With the initial disentangled representation $[\mathbf{z}_{s,1}, ..., \mathbf{z}_{s,K}]$, we can perform message-passing by aggregating neighborhood information. Let ${N_s}$ be the set of neighbors of node $v_s$. Since node $v_s$ and node $v_t \in {N_s}$ are linked due to one or two factors and could have totally dissimilar features in other factors. To avoid aggregating the noisy information from $v_s$, we will select the most similar factor for message passing. Due to the highly dependence on the homophily assumption, in homophilic graphs, the neighbor distribution of each central node is usually dominated by one specific factor according to the central node's attribute. As a result, classical GCN is powerful enough for the unitary and centralized neighbor aggregation in homophilic graph. While in the heterophilic graphs, cross-class neighborhood similarity observations given in ~\cite{ma2022is} reveal the much more complex neighbor distribution: the node connection pattern is mixed and cross-class linking is prevalent due to the existing high cross-class feature similarity. The capacity to capture and model the multiple connection patterns is thus crucial for representation learning of heterophilic graphs. Back to the disentangled learning process, for each factor, it has the potential capacity to grasp separate relation and explanation to prevent noisy aggregations when the disentanglement and independence of factors are promoted enough.Specifically, for $v_t \in {N_s}$, to improve the disentanglement, we first calculate the factor-wise importance between node $v_s$ and $v_t$ on the $k$-th factor as:
\begin{equation}
\alpha_{s, t}^{k}=\frac{\exp \left(\mathbf{z}_{s, k}^{T} \mathbf{z}_{t, k} / \tau\right)}{\sum_{i=1}^{K} \exp \left(\mathbf{z}_{s, i}^{T} \mathbf{z}_{t, i} / \tau\right)}
\label{eq:importance_normed}
\end{equation}

Following previous work ~\cite{ma2019disentangled}, the factor-wise importance value between the node s and t in the factor k is basically the similarity between a pair of transformed node features $\mathbf{z}_{s, k}$ and $\mathbf{z}_{t, k}$ in the k-th factor. The computed importance matrices is then normalized among all factors to be a measure of how well the factor k can be the explanation of the mutual relation between node s and t. $\tau$ here denotes the temperature parameter. Smaller $\tau$ will intensify the uneven degree of each factor-wise importance distribution. It will further diversify the numeric distributions of factors and promote better neighbor candidate selection for disentanglement. The computing of importance matrix can also be implemented the similar way with the attention in Graph Attention Network ~\cite{velivckovic2017graph} which is involved new parameters for training. In our module, as the original node feature $\mathbf{x}_{s}$ has been transformed to achieve the initial disentangled representations $[\mathbf{z}_{s,1}, ..., \mathbf{z}_{s,K}]$, standard Euclidean inner product for similarity has enough representation capacity to indicate the relationship between two nodes. The extra computing complexity in attention is unnecessary.

One common ground for previous works on graph disentangled learning lies in the graph neural network part: all factors share the same manner of message passing and same group of neighbors for propagation. In our framework, we propose a very simple and efficient mechanism to recast central nodes' neighbor group: 

\begin{equation}
p_{s, t}=\arg \max _{k} \alpha_{s, t}^{k}
\label{eq:max_selection}
\end{equation}

From Eq.~(\ref{eq:max_selection}), the relevance between each pair of node s and t is only allowed to participate the factor k with the largest importance value $\alpha_{s, t}^{k}$. What is the reason behind it? Some of factor-wise elements in initial transformed features $\left\{\mathbf{z}_{s, k}\right\}_{k=1}^{K}$,$\left\{\mathbf{z}_{t, k}\right\}_{k=1}^{K}$ and corresponding importance value $\left\{\alpha_{s, t}^{k}\right\}_{k=1}^{K}$ share similar numeric and structural information. It is against the expectation that a well learnt disentangled representation should be composed of a bunch of distinct factors. Many previous works add a additional discriminator to encourage the different identification on each factor. While in our method, even for factors with similar content, they will have totally different neighbor nodes for representation aggregation because node s connected with node t only participate the message passing of node t in one factor k with the largest importance value $\alpha_{s, t}^{k}$, thus the adjacency matrix of factor k's graph is:
\begin{equation}
\mathbf{A}^k=\mathbbm{1}_{p=k}\odot\mathbf{A}
\end{equation}

and the neighbor set of node s in factor k:
\begin{equation}
\mathcal{N}_{s, k}=\left\{v_{t}: v_{t} \in \mathcal{N}_{s} \wedge p_{s, t}=k\right\}
\label{eq:neighbor}
\end{equation}
Under this setting, each factor will perform message passing with the distinct node neighborhood and has $\mathbf{A}=\sum_{k=1}^{K}\mathbf{A}^{k}$. As a result, each factor only focus on its pertinent aspect of the whole graph. The far more complex underlying attribute and structural patterns in heterophilic graphs are broken down and distributed to different factor for individual explanation. This proposed neighbor selection method based on the importance matrix can effectively prevent trivial aggregations to produce the final noisy representations using the classical message passing fashion.

\subsection{Relational neighbor Aggregation Layer}
This section will introduce the detail of the aggregation scheme of our model. Utilizing the group neighbour candidates we have achieved based on Eq.~(\ref{eq:neighbor}), we perform the aggregation process as the formula to learn the representation $\mathbf{h}_{s, k}$ of node s in the factor k:
\begin{equation}
\mathbf{h}_{s, k}=\beta \mathbf{z}_{s, k}+(1-\beta) \sum_{t \in \mathcal{N}_{s, k}} \bar{\alpha}_{s, t}^{k} \mathbf{z}_{t, k}
\label{eq:layer}
\end{equation}
As shown above, no parameter for training is involved in our proposed aggregation layer which means that we implement the neural network and the propagation process separately. The input node feature $\mathbf{x}_s$ has been transformed to $\mathbf{z}_s$ in Eq.~(\ref{eq:mlp}) before the aggregation layer. We design our module in this way for several reasons. Firstly, we have managed to diversify the importance value and the central nodes' neighbors for aggregation via our proposed candidate selection approach in Eq.~(\ref{eq:importance_normed}) and Eq.~(\ref{eq:max_selection}). Adding learnable parameters after the aggregation process will recast the representations in the each factor which will lead to the decreasing of the distinguishability in these representations. Secondly, considering the complex and noisy neighborhood feature distribution in heterophilic graphs, the absence of structural information here is necessary. Independently modeling the representation of each factor only respect to the node features before the propagation step will give unmixed embeddings without the perturbation form the disassortative neighbor. The following stack of computed importance matrix based on the transformed node representation can better reflect underlying relational aspects of the targeted graph to serve as the guidance of aggregation manners for factors. Instead of creating extra computing heads for relational information besides the computing head for feature transformation in previous work \cite{velivckovic2017graph}, the learning feature can be utilized both in the importance coefficients and propagation process due to the separation structural of the proposed layer. 

The $\beta\in(0,1]$ here serves as the similar role with the teleport ratio in personalized PageRank \cite{ilprints422} to control the reservation of the information from central nodes. The preservation of this locality helps to leverage the negative influence of the disassortative contents in homophilic graphs.

For factor k, the normalization in factor-wise importance matrix in Eq.~(\ref{eq:importance_normed}) re-scale each importance value among factors to indicate its reasoning capacity towards the corresponding pair of nodes compared with other views. During the propagation, we also need to multiple the importance coefficients with corresponding node representation to maximize the the most pertinent content regarding to the central node. Another normalization in the proposed layer on all selected members in the neighborhood to balance the scale between factors is following:
\begin{equation}
\bar{\alpha}_{s, t}^{k}=\frac{\alpha_{s, t}^{k}}{\sum_{{i} \in \mathcal{N}_{s, k}} \alpha_{s, i}^{k}}
\end{equation}

\subsection{Disentangled Link Reconstruction with Self-supervised Manner}
Under the self-supervised manner, we follow the core idea of embedding learning method in the variation graph auto-encoder \cite{kipf2016variational}: given the learnt node embedding h, we rely on the link reconstruction to serve as the decoder to rich the relational information of the latent embedding. A typical process of the link reconstruction is to build the adjacency matrix depending on the learnt latent embedddings as close as the real one. A typical link reconstruction can be represented as:
\begin{equation}
\hat{\mathbf{A}}=\sigma\left(\mathbf{Z} \mathbf{Z}^{\top}\right)
\label{lr1}
\end{equation}
Since we have the factor-wise node representation including embeddings of K factors, link reconstruction in the typical manner Eq.~(\ref{lr1}) is incompatible to the disentangled learning. Intuitively, if the representation among all factors is disentangled enough, the connection between two nodes $v_s$ and $v_t$ should be mainly explained by one or two factors. If factors are incorporated together, the information from unrelated factors would disturb the reconstructed adjacency matrix. Thus, directly pooling the disentangled representation to \mathbf{H} (i.e. $\mathbf{H}=pooling\left(\left\{\mathbf{h}_{k}\right\}_{k=1}^{K}\right)$,the pooling function can be concatenation,mean,sum and etc.) as the input for link reconstruction will result mixed and noisy latent embedding with bad capacity to predict unknown structural relations. Instead of merging factors at the very beginning, we propose the disentangled link reconstruction to rebuild the adjacency matrix factor by factor following:
\begin{equation}
\hat{\mathbf{A}}_{s t}=\sigma\left(\sum_{k=1}^{K}\left(\alpha_{s, t}^{k} \mathbf{h}_{s, k}^{T} \mathbf{h}_{t, k}\right)\right)
\label{eq:re}
\end{equation}
We first factorize the link reconstruction for independent link prediction of each factor. Each factor focuses on extracting partial relational information and our candidate selection part guarantee the small overlap among factors. Therefore, when it comes to the global view of the graph, the reconstructed adjacency matrix of each factor is complementary. Combined with importance coefficient, we perform the link reconstruction as normal factor-wisely and then compute the summation of them for the overall adjacency matrix. The output goes through a non-linear function $\sigma$ such as a Sigmoid function and the attention $\alpha_{s, t}$ between connected node feature here is unnormalized:
\begin{equation}
\alpha_{s, t}^{k}=\exp \left(\mathbf{z}_{s, k}^{T} \mathbf{z}_{t, k} / \tau\right)
\end{equation}
Since the majority of pairs of nodes is unconnected, most of elements in $\mathbf{A}$ are 0. To avoid the imbalanced elements dominating the loss function, for each linked pair that  $A_{st}=1$, we sample $M$ negative pairs, i.e., $A_{sm}=0$. Here is overall loss function for the disentangled link reconstruction in our model:
\begin{equation}
\min _{\theta} \mathcal{L}_{\mathbf{A}}=\sum_{\mathbf{A}_{s t}>0}\left[\left(\hat{\mathbf{A}}_{s t}-\mathbf{A}_{s t}\right)^{2}+\frac{1}{M} \sum_{\mathbf{A}_{s m} \in \mathcal{M}_{s t}^{-}, \mathbf{A}_{s m}=0}\left(\hat{\mathbf{A}}_{s m}-\mathbf{A}_{s m}\right)^{2}\right]
\label{eq:loss}
\end{equation}
where $\theta$ is the set of parameters for the initial node representations. $M_{st}$ is the set of negative samples for $A_{st}>0$.

% change to our method
\begin{algorithm}[t]
\caption{ Training Algorithm of {\method}}
\label{alg:Framwork}
\begin{algorithmic}[1]
\REQUIRE
$\mathcal{G}=(\mathbf{V},\mathbf{A}, {X})$, $\beta$, $\tau$ and $\mathcal{M}^{-}$
\ENSURE $\theta$ of function $\left\{\mathbf{f}_{k}\right\}_{k=1}^{K}$
\WHILE{Not Converged}
\STATE Get the initial node representations $\mathbf{Z}$ via function $\left\{\mathbf{f}_{k}\right\}_{k=1}^{K}$ according to Eq.~[\ref{eq:mlp}];
\STATE Calculating the factor-wise importance matrix $\alpha$ following Eq.~[\ref{eq:importance_normed}];
\STATE Implement the neighbor selection for each factor;
\STATE Propagate $\mathbf{Z}$ via the relational neighbor aggregation Layer for embedding $\mathbf{H}$ according to Eq.~[\ref{eq:layer}];
\STATE Perform the disentangled link reconstruction for reconstructed $\hat{\mathbf{A}}$ following Eq.~[\ref{eq:re}];
\STATE Calculating the link reconstruction loss $\mathcal{L}_{\mathbf{A}}$ following Eq.~[\ref{eq:loss}];
\STATE Update $\theta$ to minimize $\mathcal{L}_{\mathbf{A}}$
\ENDWHILE
\RETURN $\theta$ 
% \RETURN  $f_P$, $f_C$, $f_G$, $\phi_{1}$ and $\phi_{2}$
\end{algorithmic}
\end{algorithm}


==> Problem_definition.tex <==
\section{Problem Definition}

% change to link prediction
We use $\mathcal{G}=(\mathcal{V}, \mathcal{E}, \mathbf{X})$ to denote an attributed graph, where $\mathcal{V}=\{v_1, ..., v_N\}$ is the set of $N$ nodes, $\mathcal{E}$ is the set of edges, and $\mathbf{X}=\{\mathbf{x_1},...,\mathbf{x_N}\}$ is the set of attributes of $\mathcal{V}$. $\mathbf{A} \in \mathbb{R}^{N \times N}$ is the adjacency matrix of the graph $\mathcal{G}$, where $\mathbf{A}_{s t}=1$ if nodes $v_s$ and $v_t$ are connected, otherwise $\mathbf{A}_{st}=0$. The links are formed due to various factors such as colleageues, common interest in music and friends relationships. However, the groundtruth of how each link is formed is unknown. Because of various latent factors causing the formation of links, the formed graph may not necessary follows homophily assumption. Directly performing message passing on such heterophilic graphs could aggregate neighbors of dissimilar features of the center nodes, causing noisy representations which degrades the performance of downstream tasks. To model the latent factors, we propose to learn disentangled latent representations of each node to capture users characteristics under each factor, which facilitate message-passing under each factor to avoid learning noisy representations. Specifically, let $K$ be the number of factors we have. $\mathbf{h}_{v,k}$ denotes the latent representations of node $v$ on factor $k$. Then the latent representation of each node $v$ will be represented as $[\mathbf{h}_{v,1},...,\mathbf{h}_{v,K}]$ for each ndoe $v$. 

==> related_work.tex <==
\subsection{Link Prediction}
Former works on link prediction utilize heuristics from the perspective of social network analysis analysis~\citep{lu2011link}. These heuristics-based approach tends to make strong assumptions and fails to generalize to the different graph structures. More seriously, they cannot effectively utilize the attribute information, which severely limits the performance of the model. With the arising of Graph Neural Networks, link prediction methods based on GNNs dominate the area since the message passing scheme can take both the structure information and the feature information~\citep{zhang2018link, kipf2016variational}. For example, VGAE makes use of latent variables and learns interpretable latent representations~\citep{kipf2016variational}. Then they use a simple inner product decoder to get the link prediction result. SEAL learns a suitable "heuristic" automatically by utilizing a mapping function between the extracted subgraphs and link existence~\cite{zhang2018link}.
\subsection{Disentangled Representation Learning}
To model the intrinsic factors in graph-structure data, there are some works that concentrate on GNNs with a disentangled model.
% DisenGCN ICML 2019
DisenGCN~\citep{ma2019disentangled} is an early-stage work and its motivation is to learn disentangled node representations and then utilize a novel neighborhood routing mechanism to find latent factors that shape the relationship between the nodes. Then for each factor, the nodes aggregate the information and get different representations.
% FactorGCN NIPS 2020
FactorGCN is similar to DisenGCN~\citep{yang2020factorizable}. First, it employs a linear layer to map the features into an embedding space. Then for each edge, it concatenates the embeddings of the nodes on the ends and feeds it into different MLP to get different edge scores and get several factor graphs. They consider an adversarial training approach to discriminate different factors and make each factor graph learn different information from the graph.
% Edge disentanglement 2022
Besides these works, \cite{zhao2022exploring} comes up with a new approach that effectively utilizes self-supervision to constrain the disentangled representations to capture distinguishable relations and neighborhood interactions.
\subsection{Graph Neural Networks for Heterophilic Graphs}
Graph Neural Networks have shown great power in learning graph representations and graph-related tasks. Graph Neural Networks have two interpretable motivations, the spectral domain motivation and the space domain motivation~\cite{hamilton2020graph}. And most of the GNNs share a message-passing architecture, which means for each node it should aggregate the information from its neighbors and then get its representation and predictions~\cite{kipf2016semi, hamilton2017inductive, velivckovic2017graph}.

GNNs have revolutionized the graph learning area, for supervised graph learning, semi-supervised learning and unsupervised graph learning. The message-passing scheme is a general approach to deal with all kinds of graph learning tasks. 
In unsupervised graph representation learning tasks, we have no labels to guide the learning process~\cite{hamilton2017representation}. For traditional network embedding methods, the supervision signal is not necessary while these approaches lack the ability of generalization~\citep{hamilton2017representation}. For graph neural networks, we should have some supervision signal to prompt GNNs to learn the graph-structure information and feature information.

Self-supervised learning gives the chance to have supervision signals for unsupervised tasks~\cite{peng2020self}. Self-supervised learning aims at extracting informative knowledge through well-designed pretext tasks without relying on manually designed labels. Self-supervision has unleashed the great potential of the rich node and edge features encoded in the graph to provide training signals. Among all the self-supervision models, contrastive learning methods alleviate the aforementioned problems and achieve state-of-the-art performance in many tasks~\cite{jin2021multi}. For instance, DGI~\cite{velickovic2019deep} employs the idea of Deep InforMax and considers both the local information and global information to provide discrimination for the contrastive module. Besides the contrastive approaches, generative and predictive approaches have also demonstrated excellent learning ability to capture the structure information and feature information~\cite{wu2021self}.

A large number of GNNs with diverse architectures have been designed. And most of the GNNs leverage message-passing to aggregate information from neighborhoods and follow the homophily assumption~\citep{zhu2020beyond}, i.e., nodes with similar features or same class labels are linked together. However, not all real-world graphs obey the homophily assumption~\citep{zheng2022graph}. There are a lot of heterophilic graphs which show the opposite property of homophilous graphs. In heterophilic graphs, linked nodes tend to have dissimilar features and different class labels. For example, in dating networks, most people tend to build a connection with people of the opposite gender~\citep{zhu2020graph}; in transaction networks, fraudsters prefer to connect with customers instead of other fraudsters~\citep{pandit2007netprobe}. And real-world graphs have more intrinsic relation information in the graph structure and are influenced by many factors.
